Dialogue State Induction Using Neural Latent Variable Models

Dialogue state modules are a useful component in a task-oriented dialogue system. Traditional methods find dialogue states by manually labeling training corpora, upon which neural models are trained. However, the labeling process can be costly, slow, error-prone, and more importantly, cannot cover the vast range of domains in real-world dialogues for customer service. We propose the task of dialogue state induction, building two neural latent variable models that mine dialogue states automatically from unlabeled customer service dialogue records. Results show that the models can effectively find meaningful slots. In addition, equipped with induced dialogue states, a state-of-the-art dialogue system gives better performance compared with not using a dialogue state module.

==> comparison-DST.tex <==
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.48\textwidth]{comparisondst.pdf}
	\caption{Comparison between DSI and traditional DST. The strikethrough font is used to represent the resources not needed by DSI. The dialogue state is accumulated as the dialogue proceeds. Turns are separated by dashed lines. Dialogues and external ontology are separated by black lines.}
	\label{fig:architecture}
\end{figure}
